On-line Viterbi Algorithm and Its Relationship to Random Walks

In this paper, we introduce the on-line Viterbi algorithm for decoding hidden Markov models (HMMs) in much smaller than linear space. Our analysis on two-state HMMs suggests that the expected maximum memory used to decode sequence of length $n$ with $m$-state HMM can be as low as $\Theta(m\log n)$, without a significant slow-down compared to the classical Viterbi algorithm. Classical Viterbi algorithm requires $O(mn)$ space, which is impractical for analysis of long DNA sequences (such as complete human genome chromosomes) and for continuous data streams. We also experimentally demonstrate the performance of the on-line Viterbi algorithm on a simple HMM for gene finding on both simulated and real DNA sequences.

==> Makefile <==
all: figures main.ps

clean:
	-rm main.aux main.bbl main.blg main.log main.log main.lot main.out \
	main.dvi main.ps main.pdf *~
	make -C figures clean

main.ps: main.dvi
	dvips main -o main.ps

main.pdf: main.dvi
	dvips -Ppdf -G0 main -o main.ps
	ps2pdf main.ps

main.dvi: figures main.tex *.tex
	latex main

bib: figures bib
	latex main
	latex main
	bibtex main
	latex main
	latex main

.PHONY: figures all bib

figures:
	make -C figures


==> data.tex <==
For the real-world data, we used 18th revision of the human genome (project?) chromosomes, 
downloaded from http://hgdownload.cse.ucsc.edu/goldenPath/hg18/chromosomes/.
These chromozomes were cut into known regions (regions that do not contain any 
unknown bases), and first 20MB of data from each of these regions were taken, 
if the region itself was at least 20MB long.
We did this in order to reduce the possibility of artifacts in the data, which could be
caused by unusually short required memory lengths for long strings of unknown bases. 

For random models, the distribution of bases was the same, as the distribution of known bases 
in the whole \#1 chromosome. 

Generated data were 20MB long sequences generated by an identical gene-finding model.

Graphs (\rref{fg:1a}\rref{fg:2a}...) show the actual memory length required at 
time $t$. Graphs (\rref{fg:1b}...) show the maximum memory up to time t, 
averaged over all 20MB sequences of corresponding type.

